MiNT: Multi-Network Training for Transfer Learning on Temporal Graphs

Temporal Graph Learning (TGL) has become a robust framework for discovering patterns in dynamic networks and predicting future interactions. While existing research has largely concentrated on learning from individual networks, this study explores the potential of learning from multiple temporal networks and its ability to transfer to unobserved networks. To achieve this, we introduce Temporal Multi-network Training MiNT, a novel pre-training approach that learns from multiple temporal networks. With a novel collection of 84 temporal transaction networks, we pre-train TGL models on up to 64 networks and assess their transferability to 20 unseen networks. Remarkably, MiNT achieves state-of-the-art results in zero-shot inference, surpassing models individually trained on each network. Our findings further demonstrate that increasing the number of pre-training networks significantly improves transfer performance. This work lays the groundwork for developing Temporal Graph Foundation Models, highlighting the significant potential of multi-network pre-training in TGL.

==> tex/08ImpactAndLimitation.tex <==
\section{Broader Impact}\label{app:impact}

Foundation models have broad applications across various domains, including the financial sector, which is our primary focus. Our goal is to develop a temporal \textcolor{black}{multi-network models capable of predicting future trends with minimal training as an initial stepping-stone toward foundation models in temporal graph}. This model can identify similar behaviors and be utilized in real-time scenarios such as network trend analysis or token price prediction \textcolor{black}{in a zero-shot setting where training a model for every new transaction network is not feasible.}. 

\textbf{Negative Impact.}
Although this work aims to pave the way for significant advancement in temporal graph learning, there might be some potential negative impacts requiring meticulous consideration.
First, the focusing on pre-training models on the TGS large collection of token transaction networks may inadvertently bias the models towards specific types of data, reducing their generalizability and effectiveness when applied to other domains or types of temporal graphs.
Second, the observed neural scaling law, which indicates that larger pre-training datasets lead to better performance, requires significant computational resources.
On one hand, extensive model pre-training leads to potential energy consumption and environmental degradation.
On the other hand, such requirements on the computational resources could lead to a concentration of advancements in well-funded institutions, potentially stifling innovation and diversity of thought in the field.
Finally, the emphasis on model performance might overshadow the importance of interpretability and transparency. Addressing these potential negative impacts is crucial to ensure the responsible development and deployment of TGL.






==> tex/ethics.tex <==
\section{Ethics and Privacy} 

All Ethereum transaction data is publicly available to users who have the necessary resources, such as fast SSDs, large RAM, and ample disk space, to synchronize Ethereum clients and manually extract blocks. Additionally, all Ethereum data is accessible on numerous Ethereum explorer sites such as \url{etherscan.io}. An Ethereum user's privacy depends on whether personally identifiable information (PII) is associated with any of their blockchain addresses, which serve as account handles and are considered pseudonymous. If such PII were obtained from other sources, our datasets could potentially be used to link Ethereum addresses. However, real-life identities can only be discovered using IP tracking information, which we neither have nor share. Our data does not contain any PII. Furthermore, we have developed a request form to exclude an address from the dataset.

==> tex/limitations.tex <==
\section{Limitations} \label{app:limitations}
Our work has the following limitations. i) Our scaling results indicate that training with a larger number of networks enhances model generalizability. Although we limited the multi-network models to sixty-four networks due to resource constraints, training on a larger number of networks could further improve performance. ii) While we used the discrete temporal directed graph setting as our benchmark, this approach can be generalized to continuous time graphs, representing a promising area for future research. iii) Although our current focus is on financial networks, the temporal scaling law should also be studied for other domains, such as social media or transportation networks, which we plan to explore in future work.
